On the Relationship Between RNN Hidden State Vectors and Semantic Ground Truth

We examine the assumption that the hidden-state vectors of recurrent neural networks (RNNs) tend to form clusters of semantically similar vectors, which we dub the clustering hypothesis. While this hypothesis has been assumed in the analysis of RNNs in recent years, its validity has not been studied thoroughly on modern neural network architectures. We examine the clustering hypothesis in the context of RNNs that were trained to recognize regular languages. This enables us to draw on perfect ground-truth automata in our evaluation, against which we can compare the RNN's accuracy and the distribution of the hidden-state vectors. We start with examining the (piecewise linear) separability of an RNN's hidden-state vectors into semantically different classes. We continue the analysis by computing clusters over the hidden-state vector space with multiple state-of-the-art unsupervised clustering approaches. We formally analyze the accuracy of computed clustering functions and the validity of the clustering hypothesis by determining whether clusters group semantically similar vectors to the same state in the ground-truth model. Our evaluation supports the validity of the clustering hypothesis in the majority of examined cases. We observed that the hidden-state vectors of well-trained RNNs are separable, and that the unsupervised clustering techniques succeed in finding clusters of similar state vectors.

==> figures/automata_table.tex <==
\begin{table}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Automata\\ name\end{tabular} &
  Description &
  \begin{tabular}[c]{@{}c@{}}Model \\ Size\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Input \\ Alphabet\\ Size\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Output \\ Alphabet\\ Size\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Characterizing \\ Set Size\end{tabular} \\ \hline
Angluin  & \begin{tabular}[c]{@{}c@{}}Accepting even number\\ of 0's and 1's\end{tabular}                               & 4  & 2  & 2  & 3 \\ \hline
Tomita 1 & -                                                                                                            & 4  & 2  & 2  & 3 \\ \hline
Tomita 3 & -                                                                                                            & 5  & 2  & 2  & 3 \\ \hline
Tomita 5 & -                                                                                                            & 4  & 2  & 2  & 3 \\ \hline
Tomita 7 & -                                                                                                            & 5  & 2  & 2  & 3 \\ \hline
Last A   & \begin{tabular}[c]{@{}c@{}}Accepting strings \\ ending with ``a''\end{tabular}                               & 2  & 2  & 2  & 1 \\ \hline
\begin{tabular}[c]{@{}c@{}}Balanced \\ Paranthases\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Accepting balanced\\ paranthases\end{tabular} &
  16 &
  2 &
  2 &
  14 \\ \hline
Regex    & \begin{tabular}[c]{@{}c@{}}Language defined by\\ {[}(({[}4-6{]}\{2\}{[}4-6{]}+)?)3{[}4-6{]}+{]}\end{tabular} & 6  & 4  & 2  & 4 \\ \hline
Mqtt     & \begin{tabular}[c]{@{}c@{}}Model of an abstacted\\ MQTT protocol\end{tabular}                                & 3  & 6  & 6  & 2 \\ \hline
TCP      & \begin{tabular}[c]{@{}c@{}}Model of a TCP\\ protocol\end{tabular}                                            & 14 & 10 & 11 & 7 \\ \hline
\end{tabular}%
}
\caption{Characteristic of finite-state automata used as a benchmark to examine RNN hidden-state space clustering.}
\label{tab:benchmark-automata}
\end{table}



==> figures/perfect_clustering_table.tex <==
\begin{table}[t]
\resizebox{\textwidth}{!}
{% \scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
\begin{tabular}[c]{@{}l@{}}Clustering Function\end{tabular} &
  \multicolumn{1}{l|}{LDA} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Logistic\\ Regression\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}DBSCAN\\ $(\epsilon=0.5$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}DBSCAN\\ $(\epsilon=0.25$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}DBSCAN\\ $(\epsilon=1.5$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}k-means\\ ($k=n$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}k-means\\ ($k=6n$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}k-means\\ ($k=8n$)\end{tabular}} &
  \multicolumn{1}{l|}{OPTICS} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}mean shift\\ ($bw=\alpha/2$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}mean shift\\ ($bw=\alpha/4$)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}mean shift\\ ($bw=\alpha/8$)\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}l@{}}\# Perfect Clustering\\ (1350 experiments)\end{tabular} &
  1003 &
  1235 &
  368 &
  185 &
  639 &
  49 &
  629 &
  783 &
  16 &
  373 &
  1296 &
  1331 \\ \hline
\begin{tabular}[c]{@{}l@{}}\# Perfect Clustering\\ (95 Experiments)\end{tabular} &
  88 &
  92 &
  80 &
  51 &
  42 &
  3 &
  90 &
  90 &
  3 &
  85 &
  93 &
  74 \\ \hline
\end{tabular}%
}
\caption{Number of perfect clustering (zero ambiguity) achieved by selected clustering method over both set of experiments.}
\label{tab:number_of_perfect_clustering}
\end{table}



==> sections/related_work_long.tex <==
In this section, we will outline the papers that, in some form or another, assume the clustering of the hidden-state space. We will focus on the parts of the presented papers that are relevant to our inquiry, and we recommend to an interested reader to further study various interesting methods presented by the papers.

Omlin and Giles~\cite{DBLP:journals/nn/OmlinG96} were amongst the first to apply principles of grammatical inference to mine rules from RNNs. More precisely, they developed an algorithm that can extract a DFA from a second-order RNN trained to recognize a regular language by applying a clustering algorithm over the RNN's hidden-state space. %(or as they call it ``a neuron space''). 
Their algorithm works on the assumption that the hidden-state space of the RNNs forms clusters, and that they correspond to the states of the automaton used to train the RNN. Furthermore, they postulate that these clusters are ``well separated'' between states of the automaton. 
%\textit{We will examine their assumption on both modern RNN architectures, as well as on larger networks compared to their seminal work.}

Zeng and Smyth~\cite{DBLP:journals/neco/ZengGS93} extended the discussion by observing that the ``clustering hypothesis'' assumed by~\cite{DBLP:journals/nn/OmlinG96} becomes unstable as longer sequences are used to extract hidden-state vectors, or as they put it ``\ldots the network forgets where the individual states are \ldots''. This is a consequence of the vanishing gradient problem, an inherent challenge of RNN training. 
%They proposed an approach to mitigate this limitation by training a network in such a way that it is stable with longer sequences. They achieve this by discretizing the hidden-state space, so that the internal representation of a state is encoded with isolated points in the hidden-state space. 
%\textit{We will examine the observations that clusters tend to intertwine for longer sequences}.   

Schellhammer et al.~\cite{DBLP:conf/conll/SchellhammerDTB98} trained an Elman RNN on a natural language processing task and constructed a state-transaction diagram representing a grammar of the data set with the help of clustering. They have performed graphical cluster analysis of the network consisting of 2 hidden neurons, thus avoiding the prepossessing (with a  dimensionality reduction technique) of hidden-state vectors as a prerequisite to visualization. They observed that activation tends to be clustered according to inputs, while data with high-frequency in the training set is dispersed in several sub-clusters. They, as well as previous approaches, managed to extract rules (encoded as a DFA) from observed clusters. It is important to note that this, as well as previous approaches, extracted a non-minimal DFA. %\textit{This could indicate that a single automaton state could be broken into several disjoint clusters. We will examine this hypothesis in our analysis.}

An empirical evaluation of rule extraction performed by Wang et al.~\cite{DBLP:journals/neco/WangZOXLG18} focused %took a closer look
on various conditions and factors that might influence DFA extraction from second-order RNNs. They empirically examined previously discussed approaches and concluded that DFAs can be ``stably'' extracted from RNN state space even when trained with short sequences. Interestingly, they observed that rules extracted from RNNs with previously outlined methods were more precise than RNNs themselves in classifying longer sequences. 
% While that might indicate that the extracted DFA is more precise than the RNN from which a DFA was extracted, we postulate that this is simply a consequence of a ``approximately correct'' DFA/rules extraction.
% That is, extracted rule set/DFA encodes input-output behavior of the RNN that conforms to the grammar used for the data set generation, while not encoding the sequences that RNN classifies. We made similar observations in~\cite{DBLP:conf/ifm/MuskardinAPT22}. \textit{More detailed discussion and examination of this assumption will be done in the future work.} 

Dong et al.~\cite{DBLP:conf/kbse/DongWSZWDDW20} combined principles from passive stochastic automata learning, namely using \textsc{Alergia}, an algorithm for the inference of Markov chains, with abstraction achieved by clustering the hidden-state space of an RNN. More precisely, they applied the k-means clustering algorithm over the hidden states observed while processing sequences from the training data set. This method mapped high-dimensional hidden-state vectors to a finite number of discrete clusters. %\textit{Clustering enabled the authors to perform adversarial data generation with the help of probabilistic verification techniques.}
% \textit{Method used in this paper prompted us to further examine the ``clustering'' hypothesis.} 

More recently, Hou and Zhou~\cite{DBLP:journals/tnn/HouZ20} extracted automata from gated RNNs with the help of clustering. They trained gated RNNs, on regular languages and a text classification task, and proposed a method similar to previously discussed ones. That is, they extract an automaton based on state transitions of the clustered hidden state space. They observed that the states indeed do cluster, and based on those clusters they construct a DFA representing the language that was used to train the RNN. They also reason about the gating mechanism and its influence on the ``clustering hypothesis''. 
%In addition, they perform visualization of a high-dimensional hidden-state space similarly as performed in Sect.~\ref{sec:analysis}. \textit{In line with their work, we will visualize and compute clusters of gated RNNs (more specifically LSTMs and GRUs) and examine how well they cluster under different conditions.}

Michalenko et al.~\cite{DBLP:conf/iclr/MichalenkoSVBCP19} examined the relationship between hidden RNN states and the states of deterministic finite automata that are used for training data generation. For this purpose, they learned functions  from the hidden state space to (sets of) automata states. They found that such functions exist, though some automata states may not to grouped in sets, 
and that linear functions appear to be sufficient.
While the existence of such functions is a positive result, the necessary
grouping of automaton states points at a weakness of the clustering hypothesis,
as it means that semantically different states cannot be distinguish in the RNN
state space. We make use of the observation that adding nonlinearity does not improve
the accuracy of these functions, thus we perform linear discriminant analysis to which we compare clusters.
%\textit{In this paper, we move one step further by not only computing such discriminant functions, but we also examine the mismatch between them and hidden state clusters derived without information about the ground truth automaton.} 



==> vertical_alg_lines.tex <==
\errorcontextlines\maxdimen



% begin vertical rule patch for algorithmicx
% borrowing from https://tex.stackexchange.com/questions/41956/marking-conditional-versions-with-line-in-margin

\RequirePackage{tikz}
\RequirePackage{zref-abspage}
\RequirePackage{zref-user}
\RequirePackage{tikz}
\RequirePackage{atbegshi}
\usetikzlibrary{calc}
\RequirePackage{tikzpagenodes}
\RequirePackage{etoolbox}

\makeatletter
\newcommand*\ALG@lastblockb{b}
\newcommand*\ALG@lastblocke{e}
\apptocmd{\ALG@beginblock}{%
    %\typeout{beginning block, nesting level \theALG@nested, line \arabic{ALG@line}}%
    \ifx\ALG@lastblock\ALG@lastblockb
        \ifnum\theALG@nested>1\relax\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi{\ALG@tikzborder}{}%
    \fi
    \let\ALG@lastblock\ALG@lastblockb%
}{}{\errmessage{failed to patch}}

\pretocmd{\ALG@endblock}{%
    %\typeout{ending block, nesting level \theALG@nested, line \arabic{ALG@line}}%
    \ifx\ALG@lastblock\ALG@lastblocke
        \addtocounter{ALG@nested}{1}%
        \addtolength\ALG@tlm{\csname ALG@ind@\theALG@nested\endcsname}%
        \ifnum\theALG@nested>1\relax\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi{\endALG@tikzborder}{}%
        \addtolength\ALG@tlm{-\csname ALG@ind@\theALG@nested\endcsname}%
        \addtocounter{ALG@nested}{-1}%
    \fi
    \let\ALG@lastblock\ALG@lastblocke%
}{}{\errmessage{failed to patch}}


\tikzset{ALG@tikzborder/.style={line width=0.5pt,black}}

\newcommand*\currenttextarea{current page text area}

\newcommand*{\updatecurrenttextarea}{%
    \if@twocolumn
        \if@firstcolumn
            \renewcommand*{\currenttextarea}{current page column 1 area}%
        \else
            \renewcommand*{\currenttextarea}{current page column 2 area}%
        \fi
    \else
        \renewcommand*\currenttextarea{current page text area}%
    \fi
}


\newcounter{ALG@tikzborder}
\newcounter{ALG@totaltikzborder}
\newenvironment{ALG@tikzborder}[1][]{%
    % Allow user to overwrite the used style locally
    \ifx&#1&\else
        \tikzset{ALG@tikzborder/.style={#1}}%
    \fi
    \stepcounter{ALG@totaltikzborder}%
    \expandafter\edef\csname ALG@ind@border@\theALG@nested\endcsname{\theALG@totaltikzborder}%
    \setcounter{ALG@tikzborder}{\csname ALG@ind@border@\theALG@nested\endcsname}%
    %\typeout{begin ALG border nesting level=\theALG@nested, tikzborder=\theALG@tikzborder, tlm=\the\ALG@tlm}%
    \tikz[overlay,remember picture] \coordinate (ALG@tikzborder-\theALG@tikzborder);% node {\theALG@tikzborder};% Modified \tikzmark macro
    \zlabel{ALG@tikzborder-begin-\theALG@tikzborder}%
    % Test if end-label is at the same page and draw first half of border if not, from start place to the end of the page
    \ifnum\zref@extract{ALG@tikzborder-begin-\theALG@tikzborder}{abspage}=\zref@extract{ALG@tikzborder-end-\theALG@tikzborder}{abspage} \else
        \updatecurrenttextarea
        \ALG@drawvline{[shift={(0pt,.5\ht\strutbox)}]ALG@tikzborder-\theALG@tikzborder}{\currenttextarea.south east}{\ALG@thistlm}%
        % If it spreads over more than two pages:
        \newcounter{ALG@tikzborderpages\theALG@tikzborder}%
        \setcounter{ALG@tikzborderpages\theALG@tikzborder}{\numexpr-\zref@extract{ALG@tikzborder-begin-\theALG@tikzborder}{abspage}+\zref@extract{ALG@tikzborder-end-\theALG@tikzborder}{abspage}}%
        \ifnum\value{ALG@tikzborderpages\theALG@tikzborder}>1
            \edef\nextcmd{\noexpand\AtBeginShipoutNext{\noexpand\ALG@tikzborderpage{\theALG@tikzborder}{\the\ALG@thistlm}}}%some pages need a border on the whole page
            \nextcmd
        \fi
    \fi
}{%
    \setcounter{ALG@tikzborder}{\csname ALG@ind@border@\theALG@nested\endcsname}%
    %\typeout{end ALG border nesting level=\theALG@nested, tikzborder=\theALG@tikzborder, tlm=\the\ALG@tlm}%
    \tikz[overlay,remember picture] \coordinate (ALG@tikzborder-end-\theALG@tikzborder);% node {\theALG@tikzborder};% Modified \tikzmark macro
    \zlabel{ALG@tikzborder-end-\theALG@tikzborder}%
    % Test if begin-label is at the same page and draw whole border if so, from start place to end place
    \updatecurrenttextarea
    \ifnum\zref@extract{ALG@tikzborder-begin-\theALG@tikzborder}{abspage}=\zref@extract{ALG@tikzborder-end-\theALG@tikzborder}{abspage}\relax
        \ALG@drawvline{[shift={(0pt,.5\ht\strutbox)}]ALG@tikzborder-\theALG@tikzborder}{ALG@tikzborder-end-\theALG@tikzborder}{\ALG@thistlm}%
    % Otherwise draw second half of border, from the top of the page to the end place
    \else
        %\settextarea
        \ALG@drawvline{\currenttextarea.north west}{ALG@tikzborder-end-\theALG@tikzborder}{\ALG@thistlm}%
    \fi
}

\newcommand*{\ALG@drawvline}[3]{%#1=from, #2=to, #3=value of \ALG@tlm/\ALG@thisthm
    \begin{tikzpicture}[overlay,remember picture]
        \draw [ALG@tikzborder]
            let \p0 = (\currenttextarea.north west), \p1=(#1), \p2 = (#2)
             in
            (#3+\fboxsep+.5\pgflinewidth+\x0,\y1+\fboxsep+.5\pgflinewidth)%-\fboxsep-.5\pgflinewidth
             --
            (#3+\fboxsep+.5\pgflinewidth+\x0,\y2-\fboxsep-.5\pgflinewidth)
            %node[midway,anchor=east] {\ALG@tikzbordertext}
        ;
    \end{tikzpicture}%
}

\newcommand{\ALG@tikzborderpage}[2]{%the whole page gets a border, #1=value of \theALG@tikzborder, #2=value of \ALG@tlm/\ALG@thistlm
    \updatecurrenttextarea
    \setcounter{ALG@tikzborder}{#1}%
    \ALG@drawvline{\currenttextarea.north west}{\currenttextarea.south east}{#2}%
    \addtocounter{ALG@tikzborderpages\theALG@tikzborder}{-1}%
    \ifnum\value{ALG@tikzborderpages\theALG@tikzborder}>1
        \AtBeginShipoutNext{\ALG@tikzborderpage{#1}{#2}}%
    \fi
    \vspace{-0.5\baselineskip}% Compensate for the generated extra space at begin of the page. No idea why exactly this happens.
}

\def\ALG@tikzbordertext{\the\ALG@tlm}
\makeatother
% end vertical rule patch for algorithmicx



% continuation indent patch, slightly extended from https://tex.stackexchange.com/questions/78776/forced-indentation-in-algorithmicx to support multiple paragraphs in one block
\RequirePackage{etoolbox}
\makeatletter
\newlength{\ALG@continueindent}
\setlength{\ALG@continueindent}{2em}
\newcommand*{\ALG@customparshape}{\parshape 2 \leftmargin \linewidth \dimexpr\ALG@tlm+\ALG@continueindent\relax \dimexpr\linewidth+\leftmargin-\ALG@tlm-\ALG@continueindent\relax}
\newcommand*{\ALG@customparshapex}{\parshape 1 \dimexpr\ALG@tlm+\ALG@continueindent\relax \dimexpr\linewidth+\leftmargin-\ALG@tlm-\ALG@continueindent\relax}
\apptocmd{\ALG@beginblock}{\ALG@customparshape\everypar{\ALG@customparshapex}}{}{\errmessage{failed to patch}}
\makeatother
% end continuation indent patch

